The Scandinavian Embedding Benchmarks: Comprehensive Assessment of Multilingual and Monolingual Text Embedding

The evaluation of English text embeddings has transitioned from evaluating a handful of datasets to broad coverage across many tasks through benchmarks such as MTEB. However, this is not the case for multilingual text embeddings due to a lack of available benchmarks. To address this problem, we introduce the Scandinavian Embedding Benchmark (SEB). SEB is a comprehensive framework that enables text embedding evaluation for Scandinavian languages across 24 tasks, 10 subtasks, and 4 task categories. Building on SEB, we evaluate more than 26 models, uncovering significant performance disparities between public and commercial solutions not previously captured by MTEB. We open-source SEB and integrate it with MTEB, thus bridging the text embedding evaluation gap for Scandinavian languages.

==> tables/coverage_domain.tex <==







\begin{table}
\centering
    \caption{Domain coverage on \gls{seb} for Mainland Scandinavian languages. The green plus (\greenplus) indicates newly added domains in \gls{seb}, while "\greenplus\greenplus" indicates that the domain was previously not covered in MTEB by any language. Black checks (\checkmark) indicate domains covered in \gls{mteb} for Scandinavian Languages, though only within translated datasets. The parenthesis is due to the LCC \cite{lcc} containing the domains, but only to a limited extent. The domains follow the categorization of the Universal Dependencies \cite{nivre-etal-2017-universal}.}
{\footnotesize
    \begin{tabular}{lcccc}
        \hline
         & \multicolumn{4}{c}{\textbf{Language}} \\ 
        \textbf{Domain} & da & nb & nn & sv \\ \hline 
        Academic & (\greenplus) & & & \\
        Bible &  & \\
        Blog &  & \\
        Fiction & \greenplus & \greenplus & \greenplus & \greenplus   \\
        Government & \greenplus\greenplus & \greenplus\greenplus & \greenplus\greenplus & \greenplus\greenplus \\
        Legal & (\greenplus\greenplus) & \greenplus\greenplus & \greenplus\greenplus &  \\
        Medical &  & & &  \\
        News & \greenplus & \greenplus & & \greenplus \\
        Non-fiction & \greenplus  & \greenplus & & \greenplus\\
        Poetry &  (\greenplus\greenplus) & & &  \\
        Reviews &  & \greenplus & &  \\
        Social & \greenplus & & & \greenplus \\
        Spoken & (\checkmark) & (\checkmark) & & (\checkmark) \\
        Wiki & \greenplus & \greenplus & \greenplus & \greenplus \\
        Web & \greenplus & &  & \greenplus\\ \hline
    \end{tabular}
    }
    \label{tab:domain_coverage}
\end{table}

==> tables/coverage_task_type.tex <==






\begin{table}[h]
\centering
\caption{Task coverage across the Scandinavian languages within \gls{seb}. The green plus (\greenplus) indicates newly added domains in \gls{seb}, while "\greenplus\greenplus" indicates that the domain was previously not covered in MTEB by any language. Black checks (\checkmark) indicate domains covered in \gls{mteb} for Scandinavian Languages, though only within translated datasets.}
{\footnotesize
\begin{tabular}{lcccc}
\hline
                                         & \multicolumn{4}{c}{\textbf{Language}} \\
\textbf{Task}                             & da & nb & nn & sv  \\  \hline
\textbf{Retrieval}                       &            &            &            &            \\
\hspace{1mm} Question answering          & \greenplus & \greenplus &            & \greenplus \\
\hspace{1mm} Article retrieval           & \greenplus\greenplus & \greenplus\greenplus &            & \greenplus\greenplus \\
\textbf{Bitext Mining}                   &            &            &            &            \\
\hspace{1mm} Dialect pairing             & \greenplus\greenplus & \greenplus\greenplus & \greenplus\greenplus & \greenplus\greenplus \\
\textbf{Classification}                  &            &            &            &            \\
\hspace{1mm} Political                   &            & \greenplus\greenplus & \greenplus\greenplus & \greenplus\greenplus \\
\hspace{1mm} Language Identification     & \greenplus & \greenplus\greenplus & \greenplus\greenplus & \greenplus\greenplus \\
\hspace{1mm} Linguistic Acceptability    & \greenplus\greenplus & \greenplus\greenplus & \greenplus\greenplus & \greenplus\greenplus \\
\hspace{1mm} Sentiment/Hate Speech       & \greenplus & \greenplus &            & \greenplus \\
\hspace{1mm} Dialog Systems              & (\checkmark) & (\checkmark) & (\checkmark) & (\checkmark) \\
\textbf{Clustering}                      &            &            &            &            \\
\hspace{1mm} Thematic Clustering         & \greenplus & \greenplus &            & \greenplus \\ \hline
\end{tabular}
}
\label{tab:task_type_coverage}
\end{table}

